A Malliavin-Gamma calculus approach to Score Based Diffusion Generative models for random fields

We adopt a Gamma and Malliavin Calculi point of view in order to generalize Score-based diffusion Generative Models (SGMs) to an infinite-dimensional abstract Hilbertian setting. Particularly, we define the forward noising process using Dirichlet forms associated to the Cameron-Martin space of Gaussian measures and Wiener chaoses; whereas by relying on an abstract time-reversal formula, we show that the score function is a Malliavin derivative and it corresponds to a conditional expectation. This allows us to generalize SGMs to the infinite-dimensional setting. Moreover, we extend existing finite-dimensional entropic convergence bounds to this Hilbertian setting by highlighting the role played by the Cameron-Martin norm in the Fisher information of the data distribution. Lastly, we specify our discussion for spherical random fields, considering as source of noise a Whittle-Mat\'ern random spherical field.

==> X2header.tex <==
%% Packages
\RequirePackage{amsthm,amsmath,amsfonts,amssymb}
\RequirePackage[numbers]{natbib}
%\RequirePackage[authoryear]{natbib}%% uncomment this for author-year citations
\RequirePackage[colorlinks,citecolor=blue,urlcolor=blue]{hyperref}%% uncomment this for coloring bibliography citations and linked URLs
%\RequirePackage{graphicx}%% uncomment this for including figures

\usepackage{a4wide} % Smaller margins
 \usepackage[ruled,linesnumbered]{algorithm2e}
\usepackage{algpseudocode}


\usepackage{makecell,multirow}
\usepackage{stmaryrd}
\DeclareMathAlphabet{\mathpzc}{OT1}{pzc}{m}{it}
\usepackage[inline]{enumitem}
\usepackage{url}
\usepackage{graphicx}
\usepackage{mathtools}
\usepackage[dvipsnames]{xcolor}\usepackage{bbm,bm}
\usepackage{mathrsfs}
%\usepackage{autonum} %faceva casini questo qua
\usepackage{makecell}
\usepackage{diagbox}
\usepackage{amssymb}
\usepackage{amsfonts}
\usepackage{upgreek}
\usepackage{nicefrac}
\usepackage{ifthen}
\usepackage{xargs}
\usepackage{caption}
\usepackage{subcaption}
\usepackage{aliascnt}
\usepackage{cleveref}
\usepackage{comment}
\usepackage{enumitem}
\usepackage{todonotes}
\newcommand{\albi}[1]{\todo[color=green!20]{{\textbf{Albi}:} #1}}
\newcommand{\giacomo}[1]{\todo[color=cyan!20]{{\textbf{Gia}:} #1}}
\newcommand{\giacomoi}[1]{\todo[color=cyan!20,inline]{{\textbf{Gia}:} #1}}
\newcommand{\gio}[1]{\todo[color=magenta!20]{{\textbf{Gio}:} #1}}
\newcommand{\verde}[1]{{\color{ForestGreen}#1}}
\newcommand{\domenico}[1]{\todo[color=yellow!20]{{\textbf{Dom}:} #1}}
\newcommand{\domenicoi}[1]{\todo[color=yellow!20,inline]{{\textbf{Dom}:} #1}}
\newcommand{\ps}[2]{\left\langle#1,#2 \right\rangle}
%% mathcal
\def\mca{\mathcal{A}}
\def\mcat{\tilde{\mathcal{A}}}
\def\mcab{\bar{\mathcal{A}}}
\def\mcb{\mathcal{B}}  %%% \mcb est déjà pris
\def\mcc{\mathcal{C}}
\def\mcy{\mathcal{Y}}
\def\mcx{\mathcal{X}}
\def\mce{\mathcal{E}}
\def\mcf{\mathcal{F}}
\def\mcg{\mathcal{G}}
\def\mch{\mathcal{H}}
\def\mcm{\mathcal{M}}
\def\mcu{\mathcal{U}}
\def\mcv{\mathcal{V}}
\def\mcr{\mathcal{R}}
\def\mcd{\mathcal{D}}
\def\mcp{\mathcal{P}}
\newcommand{\mcff}[2]{\mathcal{F}_{#1}^{#2}}
\def\mcfb{\bar{\mathcal{F}}}
\def\bmcf{\bar{\mathcal{F}}}
\def\mcft{\tilde{\mathcal{F}}}
\def\tmcf{\tilde{\mathcal{F}}}
\def\mcp{\mathcal{P}}
\def\mcq{\mathcal{Q}}
\def\mct{\mathcal{T}}
\def\cN{\mathcal{N}}
\def\FC{\mathcal{FC}^{\infty}_b}
\def\PC{\mathcal{PC}}


%%% mathsf
\def\msi{\mathsf{I}}
\def\msa{\mathsf{A}}
\def\tmsa{\tilde{\msa}}
\def\msd{\mathsf{D}}
\def\msz{\mathsf{Z}}
\def\msk{\mathsf{K}}
\def\mss{\mathsf{S}}
\def\msn{\mathsf{N}}
\def\msat{\tilde{\mathsf{A}}}
\def\msb{\mathsf{B}} 
\def\msc{\mathsf{C}}
\def\mse{\mathsf{E}}
\def\msf{\mathsf{F}}
\def\mso{\mathsf{o}}
\def\msg{\mathsf{G}}
\def\msh{\mathsf{H}}
\def\msm{\mathsf{M}}
\def\msu{\mathsf{U}}
\def\msv{\mathsf{V}}
\def\msr{\mathsf{R}}
\newcommand{\msff}[2]{\mathsf{F}_{#1}^{#2}}
\def\msp{\mathsf{P}}
\def\msq{\mathsf{Q}}
\def\msx{\mathsf{X}}
\def\msy{\mathsf{Y}}

\DeclareMathOperator{\Tr}{Tr}
\DeclareMathOperator{\Sp}{Sp}
\DeclareMathOperator{\Id}{Id}
\DeclareMathOperator{\supp}{supp}

\def\frp{\mathfrak{p}}
\def\frq{\mathfrak{q}}

\def\PE{\mathbb{E}}

\newcommand{\tcr}[1]{\textcolor{red}{#1}}
\def\plusinfty{+\infty}

\def\pistarT{\pi^{\star}}
\def\txts{\textstyle}
\def\kappamu{\kappa_{\mu}}
\def\ellmu{\ell_{\mu}}
\def\kappazeta{\kappa_{\zeta}}
\def\ellzeta{\ell_{\zeta}}
\def\rmC{\mathrm{C}}
\def\alc{\mathrm{alc}}

\def\mcpalcd{\mcp_{\alc}(\rset^d)}
\def\hatmcpalcd{\hat{\mcp}_{\alc}(\rset^d)}
\def\tmcg{\tilde{\mcg}}
\def\cmcg{\hat{\mcg}}
\def\bfW{\mathbf{W}}

\def\wiener{\mathsf{W}}

\def\rmL{\mathrm{L}}
\def\rmK{\mathrm{K}}

\def\vol{\mathrm{vol}}
\def\oo{+\infty}

\newcommand{\bes}{\begin{equation*}}
\newcommand{\ees}{\end{equation*}}
\newcommand{\beas}{\begin{eqnarray}}
\newcommand{\eeas}{\end{eqnarray}}
\newcommand{\bea}{\begin{eqnarray}}
\newcommand{\eea}{\end{eqnarray}}
\newcommand{\be}{\begin{equation}}
\newcommand{\ee}{\end{equation}}
\newcommand{\bei}{\begin{itemize}}
\newcommand{\eei}{\end{itemize}}
\newcommand{\bec}{\begin{cases}}
\newcommand{\eec}{\end{cases}}
\newcommand{\ben}{\begin{enumerate}}
\newcommand{\een}{\end{enumerate}}

\newcommand{\IND}{\mathbf{1}}
%%%%%numbersets%%%%%%%%%%
\newcommand{\bbR}{\mathbb{R}}
\newcommand{\bbRM}{\mathbb{R}^m}
\newcommand{\bbRN}{\mathbb{R}^n}
\newcommand{\bbRMN}{\mathbb{R}^{m+n}}
\newcommand{\bbRP}{\mathbb{R}_{>0}}
\newcommand{\bbRD}{\mathbb{R}^d}
\newcommand{\Sd}{\mathbb{S}^d}
\newcommand{\N}{\mathbb{N}}
\newcommand{\Z}{\mathbb{Z}}
%%%%%mathcal%%%%%%%%
\newcommand{\cA}{\mathcal{A}}
\newcommand{\cB}{\mathcal{B}}
\newcommand{\cC}{\mathcal{C}}
\newcommand{\cF}{\mathcal{F}}
\newcommand{\cE}{\mathcal{E}}
\newcommand{\cD}{\mathcal{D}}
\newcommand{\cG}{\mathcal{G}}
\newcommand{\cH}{\mathcal{H}}
\newcommand{\cI}{\mathcal{I}}
\newcommand{\cJ}{\mathcal{J}}
\newcommand{\cP}{\mathcal{P}}
\newcommand{\cY}{\mathcal{Y}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\cS}{\mathcal{S}}
\newcommand{\cT}{\mathcal{T}}
\newcommand{\cU}{\mathcal{U}}
\newcommand{\cV}{\mathcal{V}}
\newcommand{\cW}{\mathcal{W}}
\newcommand{\cL}{\mathcal{L}}
%%%%%tilde%%%%%
\newcommand{\tU}{\tilde{U}}
\newcommand{\tV}{\tilde{V}}
\newcommand{\tb}{\tilde{b}}
\newcommand{\tf}{\tilde{f}}
\newcommand{\tg}{\tilde{g}}
\newcommand{\tP}{\tilde{P}}
\newcommand{\tx}{\tilde{x}}
\newcommand{\ty}{\tilde{y}}
\newcommand{\tomega}{\tilde{\omega}}
%%%%scr%%%%%
\newcommand{\scrA}{\mathscr{A}}
\newcommand{\scrE}{\mathscr{E}}
\newcommand{\scrF}{\mathscr{F}}
%\newcommand{\scrH}{\mathscr{H}}
\newcommand{\scrH}{\mathrm{KL}}
\newcommand{\scrI}{\mathscr{I}}
\newcommand{\scrU}{\mathscr{U}}
\newcommand{\scrV}{\mathscr{V}}
\newcommand{\scrP}{\mathscr{P}}
\newcommand{\scrL}{\mathscr{L}}
%%%%%frak%%%%
\newcommand{\frkA}{\mathfrak{A}}
\newcommand{\frm}{\mathfrak{m}}

%%%%greekletters%%%%%
\newcommand{\Gm}{\Gamma}
\newcommand{\Om}{\Omega}
\newcommand{\veps}{\varepsilon}
\newcommand{\ve}{\varepsilon}
\newcommand{\vfi}{\varphi}
%%%%mathbbletters%%%%%
\newcommand{\bbD}{\mathbb{D}}
\newcommand{\bbP}{\mathbb{P}}
\newcommand{\bbE}{\mathbb{E}}
\newcommand{\bbF}{\mathbb{F}}
\newcommand{\bbQ}{\mathbb{Q}}
\newcommand{\bbS}{\mathbb{S}}
\newcommand{\bbW}{\mathbb{W}}
\newcommand{\bbX}{\mathbb{X}}
\newcommand{\bbV}{\mathbb{V}}

%%%%%boldletters%%%%%
\newcommand{\bd}{\mathbf{d}}
\newcommand{\bD}{\mathbf{D}}
\newcommand{\bE}{\mathbf{E}}
\newcommand{\bg}{\mathbf{g}}
\newcommand{\bh}{\mathbf{h}}
\newcommand{\bt}{\mathbf{t}}
\newcommand{\bff}{\mathbf{f}}
\newcommand{\bp}{\mathbf{p}}
\newcommand{\bK}{\mathbf{K}}
\newcommand{\bT}{\mathbf{T}}
\newcommand{\bP}{\mathbf{P}}
\newcommand{\bQ}{\mathbf{Q}}
\newcommand{\bR}{\mathbf{R}}
\newcommand{\bw}{\mathbf{w}}
\newcommand{\bW}{\mathbf{W}}
\newcommand{\bY}{\mathbf{Y}}
%%%%%miscellanea%%%%%
\newcommand{\Int}{[0,1]}
\newcommand{\bbl}{\begin{block}}
\newcommand{\ebl}{\end{block}}
\newcommand{\ind}{\mathbf{1}}
\newcommand{\COND}{ \big \vert}
\newcommand{\De}{\mathrm{d}}
\newcommand{\curv}{\kappa}
%%%%%%hat%%%%%%
\newcommand{\hP}{\hat{P}}
%%%rm%%%%%%%%%%
\newcommand{\rmH}{\mathrm{H}}
\newcommand{\rmI}{\mathrm{I}}
\newcommand{\rmP}{\mathrm{P}}
\newcommand{\rmQ}{\mathrm{Q}}
\newcommand{\rmR}{\mathrm{R}}
\newcommand{\rme}{\mathrm{e}}
%%%%%%bm%%%%%%%%%%%%%%%%%%%%%
\newcommand{\bmX}{\bm{X}}
\newcommand{\bmY}{\bm{Y}}
\newcommand{\bmC}{\bm{C}}
\newcommand{\bmL}{\bm{L}}
\newcommand{\bmZ}{\bm{Z}}
\newcommand{\bmu}{\bm{u}}
\newcommand{\bmw}{\bm{w}}
\newcommand{\bmf}{\bm{f}}
\newcommand{\bmQ}{\bm{Q}}



\newcommand{\vn}[1]{\left| \! \left| #1\right| \!\right|} 
\newcommand{\tn}[1]{\left| \! \left| \! \left|#1\right| \! \right| \! \right|}

\newcommand{\ip}[2]{\langle #1,#2\rangle}


\def\Lmu{L_{\mu}}
\def\Lnu{L_{\nu}}



%%%%%%%%%%%%%%%
%% alain


\def\torus{\tset}
\def\torusL{\torus_L}
\def\Haar{\mathtt{H}}
\def\HaarL{\Haar_L}

% Operands
\newcommand{\absolute}[1]{\left\vert #1 \right\vert}
\newcommand{\abs}[1]{\left\vert #1 \right\vert}
\newcommand{\absLigne}[1]{\vert #1 \vert}
\newcommand{\tvnorm}[1]{\| #1 \|_{\mathrm{TV}}}
\newcommand{\tvnormEq}[1]{\left \| #1 \right \|_{\mathrm{TV}}}
\newcommandx{\Vnorm}[2][1=V]{\| #2 \|_{#1}}
\newcommandx{\norm}[2][1=]{\ifthenelse{\equal{#1}{}}{\left\Vert #2 \right\Vert}{\left\Vert #2 \right\Vert^{#1}}}
\newcommandx{\normLigne}[2][1=]{\ifthenelse{\equal{#1}{}}{\Vert #2 \Vert}{\Vert #2\Vert^{#1}}}
\newcommand{\crochet}[1]{\left\langle#1 \right\rangle}
\newcommand{\parenthese}[1]{\left(#1 \right)}
\newcommand{\parentheseLigne}[1]{(#1 )}
\newcommand{\parentheseDeux}[1]{\left[ #1 \right]}
\newcommand{\defEns}[1]{\left\lbrace #1 \right\rbrace }
\newcommand{\defEnsLigne}[1]{\lbrace #1 \rbrace }
\newcommand{\defEnsPoint}[1]{\left\lbrace #1 \right. }
\newcommand{\defEnsPointDeux}[1]{\left. #1 \right  \rbrace }
\newcommand{\defEnsL}[1]{\left\lbrace #1 \right. }
\newcommand{\defEnsR}[1]{\left. #1 \right  \rbrace }


\def\mrl{\mathrm{L}}
\def\rml{\mrl}


\newcommand{\ensemble}[2]{\left\{#1\,:\eqsp #2\right\}}
\newcommand{\ensembleLigne}[2]{\{#1\,:\eqsp #2\}}


%% mathbb

\def\rset{\mathbb{R}}
\def\tset{\mathbb{T}}
\def\rsetd{\mathbb{R}^d}
\def\rsetdd{\mathbb{R}^{2d}}
\def\rsets{\mathbb{R}^*}
\def\cset{\mathbb{C}}
\def\zset{\mathbb{Z}}
\def\nset{\mathbb{N}}
\def\nsets{\mathbb{N}^*}
\def\qset{\mathbb{Q}}
\def\Rset{\mathbb{R}}
\def\Cset{\mathbb{C}}
\def\Zset{\mathbb{Z}}
\def\Nset{\mathbb{N}}
\def\Tset{\mathbb{T}}


\def\ie{\textit{i.e.}}
\def\cadlag{càdlàg}
\def\eqsp{\;}
\newcommand{\coint}[1]{\left[#1\right)}
\newcommand{\ocint}[1]{\left(#1\right]}
\newcommand{\ooint}[1]{\left(#1\right)}
\newcommand{\ccint}[1]{\left[#1\right]}
\newcommand{\cointLigne}[1]{[#1)}
\newcommand{\ocintLigne}[1]{(#1]}
\newcommand{\oointLigne}[1]{(#1)}
\newcommand{\ccintLigne}[1]{[#1]}
\newcommand{\cointLine}[1]{[#1)}
\newcommand{\ocintLine}[1]{(#1]}
\newcommand{\oointLine}[1]{(#1)}
\newcommand{\ccintLine}[1]{[#1]}


\def\bfm{\mathbf{m}}

\def\rmd{\mathrm{d}}
\def\Ent{\mathrm{Ent}}
\def\Leb{\mathrm{Leb}}
\def\varphistar{\varphi^\star}
\def\psistar{\psi^{\star}}
\def\pistar{\pi^{\star}}

\def\cconst{\mathrm{c}_{\mathrm{S}}}

\def\PP{\mathbb{P}}
\def\mcf{\mathcal{F}}
\def\blambda{\bar{\lambda}}
\def\blambdaV{\blambda_V}
\def\msm{\mathsf{M}}



\newcommand{\hjb}[3]{U^{{#1},{#2}}_{#3}}
\newcommand{\ent}{\mathrm{Ent}}
\def\Leb{\mathrm{Leb}}
\def\varphistar{\varphi^\star}
\def\psistar{\psi^{\star}}
\def\pistar{\pi^{\star}}


\newcommand{\sS}{{\mathbb{S}^2}}
\newcommand{\LLS}{{\rmL^2(\sS)}}
\newcommand{\cov}[2]{\operatorname{Cov}\left(#1,#2\right)}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%                                          %%
%% Uncomment next line to change            %%
%% the type of equation numbering           %%
%%                                          %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\numberwithin{equation}{section}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%                                          %%
%% For Axiom, Claim, Corollary, Hypothesis, %%
%% Lemma, Theorem, Proposition              %%
%% use \theoremstyle{plain}                 %%
%%                                          %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\theoremstyle{plain}
\newtheorem{theorem}{Theorem}
\crefname{theorem}{theorem}{Theorems}
\Crefname{Theorem}{Theorem}{Theorems}



\newaliascnt{lemma}{theorem}
\newtheorem{lemma}[lemma]{Lemma}
\aliascntresetthe{lemma}
\crefname{lemma}{lemma}{lemmas}
\Crefname{Lemma}{Lemma}{Lemmas}

\newaliascnt{corollary}{theorem}
\newtheorem{corollary}[corollary]{Corollary}
\aliascntresetthe{corollary}
\crefname{corollary}{corollary}{corollaries}
\Crefname{Corollary}{Corollary}{Corollaries}

\newaliascnt{proposition}{theorem}
\newtheorem{proposition}[proposition]{Proposition}
\aliascntresetthe{proposition}
\crefname{proposition}{proposition}{propositions}
\Crefname{Proposition}{Proposition}{Propositions}
%\newtheorem*{???}{???}
%\newtheorem{???}{???}[???]
%\newtheorem{???}[???]{???}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%                                          %%
%% For Assumption, Definition, Example,     %%
%% Notation, Property, Remark, Fact         %%
%% use \theoremstyle{remark}                %%
%%                                          %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\theoremstyle{remark}
\newtheorem{remark}{Remark}
\crefname{remark}{remark}{remarks}
\Crefname{Remark}{Remark}{Remarks}

\newaliascnt{definition}{remark}
\newtheorem{definition}[definition]{Definition}
\aliascntresetthe{definition}
\crefname{definition}{definition}{definitions}
\Crefname{Definition}{Definition}{Definitions}




\newtheorem{example}[remark]{Example}
\crefname{example}{example}{examples}
\Crefname{Example}{Example}{Examples}

\newtheorem{assumption}{\textbf{H}\hspace{-3pt}}
\Crefname{assumption}{\textbf{H}\hspace{-3pt}}{\textbf{H}\hspace{-3pt}}
\crefname{assumption}{\textbf{H}}{\textbf{H}}


\newtheorem{assumptionA}{\textbf{A}\hspace{-3pt}}
\Crefname{assumptionA}{\textbf{A}\hspace{-3pt}}{\textbf{A}\hspace{-3pt}}
\crefname{assumptionA}{\textbf{A}}{\textbf{A}}


\newtheorem{assumptionG}{\textbf{G}\hspace{-3pt}}
\Crefname{assumptionG}{\textbf{G}\hspace{-3pt}}{\textbf{G}\hspace{-3pt}}
\crefname{assumptionG}{\textbf{G}}{\textbf{G}}

\newtheorem{assumptionAO}{\textbf{AO}\hspace{-3pt}}
\Crefname{assumptionAO}{\textbf{AO}\hspace{-3pt}}{\textbf{AO}\hspace{-3pt}}
\crefname{assumptionAO}{\textbf{AO}}{\textbf{AO}}

\newtheorem{assumptionAp}{\textbf{A'}\hspace{-3pt}}
\Crefname{assumptionAp}{\textbf{A'}\hspace{-3pt}}{\textbf{A'}\hspace{-3pt}}
\crefname{assumptionAp}{\textbf{A'}}{\textbf{A'}}

%\newtheorem*{???}{???}[???]
%\newtheorem{???}[???]{???}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Please put your definitions here:        %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\newcommand{\data}{\mu_{\mathrm{data}}}
\newcommand{\fwdX}{\overrightarrow{X}}
\newcommand{\fwdalm}{\overrightarrow{a}_{\ell,m}}
\newcommand{\bwdalm}{\overleftarrow{a}_{\ell,m}}
\newcommand{\fwdM}{\overrightarrow{M}}
\newcommand{\bwdM}{\overleftarrow{M}}
\newcommand{\fwdP}{\overrightarrow{\rmP}}
\newcommand{\fwdp}{\overrightarrow{p}}
\newcommand{\bwdX}{\overleftarrow{X}}
\newcommand{\bwdP}{\overleftarrow{\rmP}}
\newcommand{\bwdp}{\overleftarrow{p}}
\newcommand{\brbr}[1]{X^{#1}}
\newcommand{\sbdm}{X^{\star}}
\newcommand{\stin}{X^{\mathrm{I}}}
\newcommand{\stinP}{\rmP^{\mathrm{I}}}
\newcommand{\stinp}{p^{\mathrm{I}}}
\newcommand{\xb}{X^{\mu,b}}
\newcommand{\Xmub}{X^{\mu,b}}
\newcommand{\fwdL}{\overrightarrow{L}}
\newcommand{\bwdL}{\overleftarrow{L}}
\newcommand{\Lou}{L^{\mathrm{OU}}}
\newcommand{\CD}{\mathrm{CD}}
